A Vertex-Weighted Tutte Symmetric Function, and Constructing Graphs with Equal Chromatic Symmetric Function

This paper has two main parts. First, we consider the Tutte symmetric function $XB$, a generalization of the chromatic symmetric function. We introduce a vertex-weighted version of $XB$ and show that this function admits a deletion-contraction relation. We also demonstrate that the vertex-weighted $XB$ admits spanning-tree and spanning-forest expansions generalizing those of the Tutte polynomial by connecting $XB$ to other graph functions. Second, we give several methods for constructing nonisomorphic graphs with equal chromatic and Tutte symmetric functions, and use them to provide specific examples.

==> bibThesis.tex <==
\bibitem{per} Alexandersson, Per, and Greta Panova. ``LLT polynomials, chromatic quasisymmetric functions and graphs with cycles." Discrete Mathematics 341.12 (2018): 3453--3482.

\bibitem{trees} Aliste-Prieto, Jos\'e, Anna de Mier, and Jos\'e Zamora. ``On trees with the same restricted U-polynomial and the Prouhet-Tarry-Escott problem." Discrete Mathematics 340.6 (2017): 1435--1441.

\bibitem{birk} Birkhoff, George D. ``A determinant formula for the number of ways of coloring a map." The Annals of Mathematics 14.1/4 (1912): 42--46.

\bibitem{huh} Cho, Soojin, and JiSun Huh. ``On $ e $-positivity and $ e $-unimodality of chromatic quasisymmetric functions." arXiv preprint arXiv:1711.07152 (2017).

\bibitem{cho} Cho, Soojin, and Stephanie van Willigenburg. ``Chromatic classical symmetric functions." arXiv preprint arXiv:1604.03954 (2016).

\bibitem{chow} Chow, Timothy Y. ``The path-cycle symmetric function of a digraph." Advances in Mathematics 118.1 (1996): 71--98.

\bibitem{cs} Crew, Logan, and Sophie Spirkl. ``A Deletion-Contraction Relation for the Chromatic Symmetric Function." arXiv preprint arXiv:1910.11859 (2019).

\bibitem{data} Crew, Logan, and Sophie Spirkl. ``Examples of Pairs of Small Graphs with Equal Chromatic Symmetric Function''. Logan Crew's Homepage. Google Sites, https://sites.google.com/site/ltcrewmath/exampl.pdf. PDF download.

\bibitem{paper} Crew, Logan, and Sophie Spirkl.  ``Using Deletion-Contraction to Construct Graphs with Equal Chromatic Symmetric Function''. In preparation.

\bibitem{epos} Dahlberg, Samantha, Adrian She, and Stephanie van Willigenburg. ``Schur and $ e $-positivity of trees and cut vertices." arXiv preprint arXiv:1901.02468 (2019).

\bibitem{dahl} Dahlberg, Samantha, and Stephanie van Willigenburg. ``Lollipop and lariat symmetric functions." SIAM Journal on Discrete Mathematics 32.2 (2018): 1029--1039.

\bibitem{ell} Ellzey, Brittney. ``A directed graph generalization of chromatic quasisymmetric functions." arXiv preprint arXiv:1709.00454 (2017).

\bibitem{fayers} Fayers, Matthew. ``A note on Kostka numbers." arXiv preprint arXiv:1903.12499 (2019).


\bibitem{foley} Foley, Ang\`ele M., Ch\'\i nh T. Ho\`ang, and Owen D. Merkel. ``Classes of graphs with e-positive chromatic symmetric function." Electronic Journal of Combinatorics 26.3 (2019): P3--51.

\bibitem{gash} Gasharov, Vesselin. ``Incomparability graphs of (3+1)-free posets are s-positive." Discrete Mathematics 157.1--3 (1996): 193--197.

\bibitem{noncomm} Gebhard, David D., and Bruce E. Sagan. ``A chromatic symmetric function in noncommuting variables." Journal of Algebraic Combinatorics 13.3 (2001): 227--255.

\bibitem{grin} Grinberg, Darij. ``Double Posets and the Antipode of QSym." Electronic Journal of Combinatorics 24.2 (2017): P2--22.

\bibitem{guay} Guay-Paquet, Mathieu. ``A modular relation for the chromatic symmetric functions of (3+1)-free posets." arXiv preprint arXiv:1306.2400 (2013).

\bibitem{hamel} Hamel, Ang\`ele M., Ch\'\i nh T. Ho\`ang, and Jake E. Tuero. ``Chromatic symmetric functions and H-free graphs." Graphs and Combinatorics 35.4 (2019): 815--825.

\bibitem{hasebe} Hasebe, Takahiro, and Shuhei Tsujie. ``Order quasisymmetric functions distinguish rooted trees." Journal of Algebraic Combinatorics 46.3--4 (2017): 499--515.

\bibitem{heil} Heil, Sam, and Caleb Ji. ``On an Algorithm for Comparing the Chromatic Symmetric Functions of Trees." arXiv preprint arXiv:1801.07363 (2018).

\bibitem{kaz} Kaliszewski, Ryan. ``Hook coefficients of chromatic functions." arXiv preprint arXiv:1404.7531 (2014).

\bibitem{umbra} Lenart, Cristian, and Nigel Ray. ``Chromatic polynomials of partition systems." Discrete Mathematics 167 (1997): 419--444.

\bibitem{mac} Macdonald, Ian Grant. ``Symmetric functions and Hall polynomials.'' Oxford University Press (1998).

\bibitem {martin} Martin, Jeremy L., Matthew Morin, and Jennifer D. Wagner. ``On distinguishing trees by their chromatic symmetric functions." Journal of Combinatorial Theory, Series A 115.2 (2008): 237--253.

\bibitem{martin2} Martin, Jeremy L., and Jennifer D. Wagner. ``On the chromatic symmetric function of a tree." Extended abstract for 18th Annual Conference on Formal Power Series and Algebraic Combinatorics, San Diego. 2006.

\bibitem{mckay} McKay, Brendan. ``Combinatorial Data''. Brendan McKay's Home Page. Australian National University, users.cecs.anu.edu.au/{\raise.17ex\hbox{$\scriptstyle\sim$}}bdm/data/. 

\bibitem{ore} Orellana, Rosa, and Geoffrey Scott. ``Graphs with equal chromatic symmetric functions." Discrete Mathematics 320 (2014): 1--14.

\bibitem{pau} Paunov, Alexander. ``Planar graphs and Stanley's Chromatic Functions." arXiv preprint arXiv:1702.05787 (2017).

\bibitem{paw} Pawlowski, Brendan. ``Chromatic symmetric functions via the group algebra of $S_n$." arXiv preprint arXiv:1802.05470 (2018).

\bibitem{ray2} Ray, Nigel, and Colin Wright. ``Umbral interpolation and the addition/contraction tree for graphs." Discrete Mathematics 103.1 (1992): 67--74.

\bibitem{sagan} Sagan, Bruce E. ``The symmetric group: representations, combinatorial algorithms, and symmetric functions.'' Vol. 203. Springer Science \& Business Media, 2013.

\bibitem{acyc} Stanley, Richard P. ``Acyclic orientations of graphs." Discrete Mathematics 5.2 (1973): 171--178.

\bibitem{stanley} Stanley, Richard P. ``A symmetric function generalization of the chromatic polynomial of a graph." Advances in Mathematics 111.1 (1995): 166--194.

\bibitem{stanleybook1} Stanley, Richard P. ``Enumerative Combinatorics Volume 1 second edition." Cambridge Studies in Advanced Mathematics (2011).

\bibitem{stanleybook} Stanley, Richard P. ``Enumerative Combinatorics, Vol. 2." Cambridge Studies in Advanced Mathematics (1999).


\bibitem{wachs} Shareshian, John, and Michelle L. Wachs. ``Chromatic quasisymmetric functions." Advances in Mathematics 295 (2016): 497--551.

\bibitem{tsu} Tsujie, Shuhei. ``The chromatic symmetric functions of trivially perfect graphs and cographs." Graphs and Combinatorics 34.5 (2018): 1037--1048.

\bibitem{wang} Wang, David G.L., and Monica M.Y. Wang. ``Non-Schur-positivity of chromatic symmetric functions." arXiv preprint arXiv:2001.00181 (2020).

\bibitem{wolfgang} Wolfgang, Harry Lewis. ``Two interactions between combinatorics and representation theory: monomial immanants and Hochschild cohomology.'' Diss. Massachusetts Institute of Technology, 1997.

